GraspGPT: Leveraging Semantic Knowledge from a Large Language Model for Task-Oriented Grasping

Task-oriented grasping (TOG) refers to the problem of predicting grasps on an object that enable subsequent manipulation tasks. To model the complex relationships between objects, tasks, and grasps, existing methods incorporate semantic knowledge as priors into TOG pipelines. However, the existing semantic knowledge is typically constructed based on closed-world concept sets, restraining the generalization to novel concepts out of the pre-defined sets. To address this issue, we propose GraspGPT, a large language model (LLM) based TOG framework that leverages the open-end semantic knowledge from an LLM to achieve zero-shot generalization to novel concepts. We conduct experiments on Language Augmented TaskGrasp (LA-TaskGrasp) dataset and demonstrate that GraspGPT outperforms existing TOG methods on different held-out settings when generalizing to novel concepts out of the training set. The effectiveness of GraspGPT is further validated in real-robot experiments. Our code, data, appendix, and video are publicly available at https://sites.google.com/view/graspgpt/.

==> data.tex <==
\section{Problem Formulation}
We consider the problem of estimating the posterior distribution $P(G^*|O,I)$ given an object point cloud $O$ and a language instruction $I$ specifying the target object class and the target task (e.g., ``Use the \textit{knife} to \textit{cut}" and ``to \textit{drink}, grasp the \textit{mug}"), where $G^*$ is the space of all task-oriented grasps. Each grasp $g \in G^*$ is a parallel-jaw gripper pose $(R, T)$ given in $SE(3)$,  where $R \in SO(3)$ is the 3D orientation and $T \in \mathbb{R}^3$ is the 3D translation of the gripper. To ensure the generalization to novel concepts, we incorporate the semantic knowledge from an LLM $P(G^*|O,I,D)$, where $D$ is language descriptions of the concepts.

Following the convention in previous work \cite{murali2021same}, \textcolor{red}{we factorize the estimation process into two steps:} (1) task-agnostic grasp sampling $P(G|O)$, and (2) task-oriented grasp evaluation $P(S|O, I, D, g)$, where $S$ is the probability of success for $g$. Since the first step is well-studied by prior works\cite{ten2018using}\cite{mousavian20196}, we assume the access to a set of stable task-agnostic grasp candidates and focus on the second step.

\section{Data Generation}\label{data}

\subsection{Description Generation}
\subsection{Instruction Generation}








